WarpDiffusion: Efficient Diffusion Model for High-Fidelity Virtual Try-on

Image-based Virtual Try-On (VITON) aims to transfer an in-shop garment image onto a target person. While existing methods focus on warping the garment to fit the body pose, they often overlook the synthesis quality around the garment-skin boundary and realistic effects like wrinkles and shadows on the warped garments. These limitations greatly reduce the realism of the generated results and hinder the practical application of VITON techniques. Leveraging the notable success of diffusion-based models in cross-modal image synthesis, some recent diffusion-based methods have ventured to tackle this issue. However, they tend to either consume a significant amount of training resources or struggle to achieve realistic try-on effects and retain garment details. For efficient and high-fidelity VITON, we propose WarpDiffusion, which bridges the warping-based and diffusion-based paradigms via a novel informative and local garment feature attention mechanism. Specifically, WarpDiffusion incorporates local texture attention to reduce resource consumption and uses a novel auto-mask module that effectively retains only the critical areas of the warped garment while disregarding unrealistic or erroneous portions. Notably, WarpDiffusion can be integrated as a plug-and-play component into existing VITON methodologies, elevating their synthesis quality. Extensive experiments on high-resolution VITON benchmarks and an in-the-wild test set demonstrate the superiority of WarpDiffusion, surpassing state-of-the-art methods both qualitatively and quantitatively.

==> figures/teaser1.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\hsize]{figures/teaser.pdf}
  \vspace{-4mm}
  \caption{Our WarpDiffusion can generate high-fidelity try-on results with photo-realistic 3D-aware effects like wrinkles and shadows.}
   \vspace{-4mm}
  \label{fig:teaser}
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
Image-based Virtual Try-On (VITON) aims to transfer an in-shop garment image onto a target person. While existing methods focus on warping the garment to fit the body pose, they often overlook the synthesis quality around the garment-skin boundary and realistic effects like wrinkles and shadows on the warped garments. These limitations greatly reduce the realism of the generated results and hinder the practical application of VITON techniques. Leveraging the notable success of diffusion-based 
models in cross-modal image synthesis, some recent diffusion-based methods have ventured to tackle this issue. However, they tend to either consume a significant amount of training resources or struggle to achieve realistic try-on effects and retain garment details. For efficient and high-fidelity VITON, we propose WarpDiffusion, which bridges the warping-based and diffusion-based paradigms via a novel informative and local garment feature attention mechanism. Specifically, WarpDiffusion incorporates local texture attention to reduce resource consumption and uses a novel auto-mask module that effectively retains only the critical areas of the warped garment while disregarding unrealistic or erroneous portions. Notably, WarpDiffusion can be integrated as a plug-and-play component into existing VITON methodologies, elevating their synthesis quality. Extensive experiments on high-resolution VITON benchmarks and an in-the-wild test set demonstrate the superiority of WarpDiffusion, surpassing state-of-the-art methods both qualitatively and quantitatively. 




%While diffusion-based models  have recently achieved remarkable success in cross-modal image synthesis, 
%these models are not specifically designed for VITON and the resource consumption for training these models is often prohibitive.
%Recently, diffusion-based models such as Midjourney and StableDiffusion have achieved remarkable success in cross-modal image synthesis. However, none of these models are specifically designed for VITON, and the resource consumption for training these models is often unaffordable.
 %to leverage the powerful generative ability of diffusion models for the VITON task.WarpDiffusion can seamlessly be integrated as a plug-and-play component into existing VITON methodologies, elevating their synthesis quality
%WarpDiffusion incorporates local texture attention to reduce resource consumption. 

%\zfd{should clarify the importance of auto-mask module. rephrase "deserving attention"?}
%\Zxj{should polish this words I'm not sure}
%Moreover, WarpDiffusion proposes a novel auto-mask module, that effectively retains the most critical areas of the warped garment, thereby enhancing its 3D-aware effects. '


% \zfw{FYI: To hide all comments (except Xujie's which I cannot find where it is defined), just uncomment the $\backslash commentsfalse$ in main.tex.}
%Furthermore, the versatility of our method is evident in results obtained across different warp garments, reaffirming its efficacy in diverse scenarios.

%Additionally, WarpDiffusion introduces
%a novel \xd{give a name} module 
%a novel auto mask module to effectively determine the parts of a warped garment that deserve attention, which can enhance the 3D-aware effects of the warped garment
%to extract texture information\xd{extract texture is nothing new, try to merge with later sentences and highlight our contribution} . It collaboratively combines global and local information to guide the try-on denoising process.
%Furthermore, WarpDiffusion can be easily integrated as a plug-and-play components
%\xd{previously you mention windows attention and module, here you cannot call it as module. Otherwise, you repharse previous sentences}
%into existing VITON methods to improve their synthesis quality.
%Extensive experiments conducted on two high-resolution VITON benchmarks demonstrate that WarpDiffusion outperforms existing state-of-the-art methods both qualitatively and quantitatively. Moreover,the results obtained using different warp garments demonstrate the versatility of our method.
%\xd{any quantitative comparisons or results about ``cost-effective" during training/inference. And have you plugged your modules into more than one VITON module or SD backbone? if not, the plug-and-play maybe questioned}

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}

Virtual Try-On (VITON) is gaining significant traction in the e-commerce industry due to its potential to revolutionize online shopping with virtual changing room experiences.
VITON achieves this by generating highly realistic images of a person wearing a specific garment from an in-shop garment image and a person image~\cite{han2018viton}.
However, most existing approaches fail to meet the following synthesis quality requirements of today’s e-commerce scenarios:
1) \textbf{Accurate Garment Deformation}: The provided garment should be precisely deformed to fit the body pose of the target person, while preserving garment characteristics such as shape and texture. 
2) \textbf{Realistic Try-On Effect}: The synthesized results should not only preserve the inherent characteristics of the garment but also incorporate realistic try-on effect, including wrinkles and shadows on the garment region;
3) \textbf{Consistent Visual Quality}: The visual quality of the results should be consistently high throughout the entire image, without any noticeable artifacts or blurriness in local regions such as the skin-garment boundary or neck region. 

Most existing methods~\cite{wang2018toward,yang2020towards,ge2021parser,lee2022high,xie2023gp} employ a two-stage framework for try-on synthesis. In the first stage, a neural network is used to model the explicit deformation field, via a Thin Plate Spline (TPS) transformation~\cite{bookstein1989principal} or appearance flow~\cite{zhou2016view}, for garment warping. In the second stage, Generative Adversarial Networks (GANs)~\cite{goodfellow2014generative} are used for try-on synthesis.
However, these two-stage methods heavily rely on the warping module and often fail to meet the above-mentioned synthesis quality requirements. Specifically, the explicit deformation field used in the first stage often struggles to handle complex non-rigid deformations, which can negatively impact the subsequent try-on synthesis. For instance, in the first row of Fig~\ref{fig:teaser}, when the designated person has a challenging body pose, such as crossed arms, baselines~\cite{he2022style,xie2023gp,bai2022single,ge2021parser,gou2023taming} all show excessive distortion where the arms intersect.

Besides, since the explicit deformation field directly performs warping in pixel space, the try-on appearance is solely determined by the original in-shop garment. As shown in the second row of Fig.~\ref{fig:teaser}, when the given garment is a flat image without any realistic wrinkles or shadows, these methods are unable to produce realistic results. 

Furthermore, due to the limited training data and training instability, GAN-based generators struggle to learn the specific distribution for fine details, resulting in inferior synthesis quality for certain local regions. For instance, these methods often generate blurry or jagged artifacts around the skin-garment boundary, which is evident in the third row of Fig.~\ref{fig:teaser}.  Further, none of the prior approaches are able to accurately capture the see-through nature of the garment in the belly region in this example.

Recently, in light of the significant success of diffusion models for image synthesis, some pioneering methods~\cite{huang2023composer,chen2023anydoor} have attempted to explore the application of diffusion models to VITON. However, these methods do not incorporate any deformation mechanism, which leads to spatial misalignment between the in-shop garment and body pose, ultimately resulting in a loss of garment details.
\begin{table}[t]
\def\arraystretch{1.2}
\small
\tabcolsep 6pt
\centering
\begin{tabular}{c c c c c c }
  \toprule
    \multicolumn{2}{c}{Method}                              
  & & Devices & Training time & Data \\
  \cmidrule{1-2} \cmidrule{4-6}  
  \multicolumn{2}{c}{TryonDiffusion\cite{zhu2023tryondiffusion}} 
  & & 32 TPU-v4 & 9 Days & 4M   \\
  \multicolumn{2}{c}{WarpDiffusion} 
  & & 8 A100 & 1 Day & 30K  \\ 
  \bottomrule
\end{tabular}
\caption{WarpDiffusion requires significantly less training resources than TryonDiffusion~\cite{zhu2023tryondiffusion}. }
\vspace{-6mm}
\label{tab:training}
\end{table}
To resolve this issue, TryOnDiffusion~\cite{zhu2023tryondiffusion} introduces an implicit deformation field via cross-attention layers~\cite{vaswani2017attention} to warp the input garment. However, while this approach leads to a scalable model for high-fidelity try-on synthesis, its training requires a prohibitive amount of resources, including 4 million paired data samples and thousands of GPU hours.

In order to leverage the generative capabilities of diffusion models for the VITON task in the face of limited resources, we introduce a novel effective and efficient model called WarpDiffusion in this work. WarpDiffusion combines the efficiency of explicit warping modules 
with the generative capability of pre-trained text-to-image diffusion models (i.e., StableDiffusion~\cite{rombach2022high}) to achieve high-fidelity try-on synthesis. It is worth noting that this bridging is not trivial and previous attempts fail to preserve garment details~\cite{gou2023taming,morelli2023ladi}. 
We solved this by introducing a novel informative and local garment feature attention mechanism that ensures accurate garment deformation and synthesis of realistic effects, while addressing the imperfections of the explicit warping results.
%We solved this by introducing a novel informative and local garment feature attention mechanism to ensure accurate garment deformation and realistic effect, handling with the imperfection of the explicit warping results. 
Meanwhile, this mechanism introduces almost no overhead when compared to the original StableDiffusion model. As shown in Table~\ref{tab:training}, the entire model can be trained on 8 NVIDIA A100 GPUs at a resolution of 1024, with a significantly lower training consumption than that of TryonDiffusion~\cite{zhu2023tryondiffusion}. Furthermore, our WarpDiffusion is not reliant on a specific warping module and can be seamlessly integrated as a plug-and-play module into previous GAN-based try-on methods~\cite{ge2021parser,he2022style,bai2022single,xie2023gp}. 

%\xiu{above is fine}

 % Our goal is to extract texture directly from the garment, while generates 3D details like wrinkles from real data distributions.To address these complexities, WarpDiffusion introduces an innovative auto mask module. This module efficiently generates an enhanced warped garment, focusing the model on crucial garment details \zfw{like ...?}. This ensures not only texture consistency but also fosters the creation of more authentic 3D awareness. 


\begin{figure*}[t]
  \centering
  \includegraphics[ width=1.0\textwidth]{figures/framework_final_v3.pdf}
  \caption{The framework of our WarpDiffusion. During the training stage, the garment-agnostic image $I_a$, garment-agnostic mask $M_a$, skin mask $M_s$, and foreground mask $M_f$ are concatenated with the input noise $I'_t$ and injected into the diffusion UNet. The in-shop garment $G$ is extracted via the Global Garment Feature Encoder and used in the cross-attention. Simultaneously, the warped garment $G_w$ and the warped garment mask $M_w$ are processed by the Auto Mask module to obtain an informative mask $M_\text{info}$. $M_\text{info}$ is then used to derive an improved warped garment, denoted as $G'_w$, which is subsequently utilized in the local texture attention. During the inference step, we employ the warped result from any try-on model to generate realistic try-on results, showcasing WarpDiffusion's plug-and-play capability.}
\vspace{-4mm}

  \label{fig:framework}
\end{figure*}



%The entire model can be trained on 4 NVIDIA A100 GPUs at the resolution of 1024 while ensuring model complexity and model performance.As show in table ~\ref{tab:training},it's less than TryonDiffusion\cite{zhu2023tryondiffusion} with a large margin\Zxj{maybe put train table \ref{tab:training} here?} \commentM{Yes, I think that makes sense. You can still link back to it when you talk about it in the method section, but it clearly highlights one of the benefits.}

%To be specific, WarpDiffusion first employs the previous warping module~\cite{Ge2021PFAFN,he2022fs_vton,xie2023gpvton} to deform the in-shop garment, then a latent diffusion model is used to integrate the warped garment and the original garment-agnostic person information to obtain the try-on results. 
%For the latent diffusion model, WarpDiffusion leverages the pre-trained StableDiffuion for network initialization, which can inherit the generation prior and speed up the network convergence. 
%Specifically, WarpDiffusion first utilizes a warping module~\cite{Ge2021PFAFN,he2022fs_vton,xie2023gpvton}) to deform the in-shop garment. Then, a latent diffusion model is employed to integrate the warped garment with the original garment-agnostic person information, resulting in the try-on results.\xd{leave these to method, try to make introduction short and interesting}
%For the latent diffusion model, WarpDiffusion leverages the pre-trained StableDiffusion for network initialization, allowing it to inherit the generation prior and expedite network convergence.
%Additionally,to enhance the model's focus on vital regions of the warped garment, we introduce a novel auto mask module. This module directs the model's attention to the crucial information of the garment, ensuring texture consistency and facilitating the generation of more authentic 3D-awareness.finally  WarpDiffusion combines unwarped and warped garment information to guide the denoising process. The unwarped cloth encompasses high-level garment characteristics such as shape, color, and coarse-grain patterns, ensuring accurate denoising even in complex scenarios where the warped garment may be distorted. The warped garment information, which is well aligned with the body pose, is used to guide the generation of texture details
%Even if the warping result contains noise or excessive distortion, WarpDiffusion can still fix it and improve the quality and the Realism of the try-on result.
%To reduce memory usage, the local warped garment is passed through a VAE encoder and then sent to the cross-attention layer using custom-designed window attention.
%This approach maximizes the retention of clothing information without excessive feature compression, enabling informative clothing features to guide texture details.
%Besides, WarpDiffusion jointly employs global and local garment information to guide the denoising process, in which the two kinds of information are derived from the in-shop garment and the warped garment, respectively. 
%The global information refers to the high-level information of the garment (e.g., shape, color, coarse-grain pattern, etc.), which can guarantee accurate denoising even when the warped garment is broken in some complicated cases.
 %the warped garment is sent to the cross attention layer through a vae encoder. We use customlize-window attention to reduce the memory usage. This allows us to retain the clothing features to the maximum extent without having to compress the features too much. as a result，an informative clothing feature can provide guidance about texture details.


%However, as mentioned above, directly using the guidance of warped garment will lead to inferior results and lack of 3D-aware effects. To alleviate the heavy reliance on the warped garment, WarpDiffusion introduces a novel auto mask network whick is jointly trained with diffusion model to extract the texture information from the warped garment. 
%Specifically, the auto mask network applies the Unet to extract the most useful information from the warped garment feature, which will then provide the local guidance for the diffusion network.
%Since the feature after automask network only contains the principal information of the garment texture (e.g., logo, pattern, etc.), the diffusion network is forced to utilize the global information for complete garment synthesis and has the potential to learn the 3D-aware pattern from the real data distribution.
%Furthermore, since WarpDiffusion does not rely on the particular warping module, it can serve as a plug-and-play module for previous GAN-based try-on methods~\cite{Ge2021PFAFN,he2022fs_vton,bai2022sdafn,xie2023gpvton} to consistently improve the quality of the try-on results.

%Overall, our contributions can be concluded as follows: 
%(1) We propose a warping and diffusion intergraded framework, named WarpDiffusion, to collaboratively employ global and local garment information for high-fidelity virtual try-on synthesis in real-world scenarios . 
%(2) WarpDiffusion utilizes the pre-trained StableDiffusion and custom-designed windows attention specifically for initialization conditions. This approach enhances the synthesis quality of the body region and significantly minimizes resource consumption during network training.
%(3) WarpDiffusion introduces a novel auto mask network %high-frequency extractor
%to extract the texture information for try-on generation, which can facilitate the synthesis of 3D-aware patterns like wrinkles and shadows.
%(4) Extensive experiments on the public try-on benchmarks and in-the-wild test set demonstrate that WarpDiffsuion outperforms existing SOTAs and can serve as a plug-and-play module to improve the synthesis quality of existing methods.
Overall, our contributions can be summarized as follows:
\begin{itemize}
    \item We propose WarpDiffusion, a framework integrating both explicit warping and a diffusion model, to collaboratively utilize global and local garment information for high-fidelity VITON synthesis in real-world scenarios.
    %We propose WarpDiffusion, a warping and diffusion integrated framework, to collaboratively utilize global and local garment information for high-fidelity virtual try-on synthesis in real-world scenarios.
    \item  WarpDiffusion leverages the pre-trained StableDiffusion and a custom-designed local texture attention to enhance the synthesis quality of the body region and significantly reduces resource consumption during training.
    \item WarpDiffusion introduces a novel Auto Mask Module for informative garment feature extraction, enabling the synthesis of realistic try-on effects such as wrinkles and shadows without loss of details.
    %WarpDiffusion introduces a novel auto mask module to keep import information on the warped garment for try-on generation, enabling the synthesis of 3D-aware patterns such as wrinkles and shadows.
    \item Extensive experiments conducted on public try-on benchmarks and in-the-wild test sets demonstrate that WarpDiffusion outperforms existing state-of-the-art methods and can be easily integrated as a plug-and-play module to enhance the synthesis quality of existing approaches.
\end{itemize}




